DefGraspSim: Simulation-based grasping of 3D deformable objects

Robotic grasping of 3D deformable objects (e.g., fruits/vegetables, internal organs, bottles/boxes) is critical for real-world applications such as food processing, robotic surgery, and household automation. However, developing grasp strategies for such objects is uniquely challenging. In this work, we efficiently simulate grasps on a wide range of 3D deformable objects using a GPU-based implementation of the corotational finite element method (FEM). To facilitate future research, we open-source our simulated dataset (34 objects, 1e5 Pa elasticity range, 6800 grasp evaluations, 1.1M grasp measurements), as well as a code repository that allows researchers to run our full FEM-based grasp evaluation pipeline on arbitrary 3D object models of their choice. We also provide a detailed analysis on 6 object primitives. For each primitive, we methodically describe the effects of different grasp strategies, compute a set of performance metrics (e.g., deformation, stress) that fully capture the object response, and identify simple grasp features (e.g., gripper displacement, contact area) measurable by robots prior to pickup and predictive of these performance metrics. Finally, we demonstrate good correspondence between grasps on simulated objects and their real-world counterparts.

==> old_section_8.tex <==
\section{Application to Unseen Objects (OLD)}
\vspace{-3pt}
% Moved to section 7, comment out 
% In Section~\ref{primitives}, for each primitive object, the 7 features and 7 performance metrics are evaluated for all grasps. For each metric, one random forest classifier is trained. The input to each classifier is the features of a grasp in the 30th percentile of either end of the distribution of all grasps ranked by their metric, and the output prediction is whether the grasp belongs to the higher or lower range.
% \YN{Are the inputs to the classifier only the grasp features that correspond to the grasps that are \textit{actually} within the top or bottom 30th percentile? In other words, do we train or test on grasps that are, e.g., in the 50th percentile?}\IH{yeah, the inputs are only the top and bottom 30, I can edit to make more clear} 
We first test whether the classifiers trained in Section~\ref{primitives} immediately generalize by applying them to candidate grasps on unseen real-world objects (gray objects in Fig.~\ref{fig:object_categories}). Performance was limited due to overfitting caused by the small number of primitives and grasps used in training.
% Performance is found to be inadequate due to the small number of primitive geometries examined and limited size of the training set. \IH{potentially removable bc we don't really explain it, or moving this to limitations. How to motivate using just one feature? As a first step towards transferring a learned model from primitives to substantially different unseen objects}\IH{although dataset is large, limited by number of primitives and number of grasps used in training}
%even when the tested classifiers are trained on primitives geometrically similar to the unseen objects
% \IH{smooth out transition. Concept of overfitting -> immediately obvious why you would go down to lower dimension}
We thus reduce the dimensionality by using \textit{one} grasp feature instead of seven, which is suitable when there is only one dominantly informative feature.
% We instead opt for the following simplified approach: 
% rather than using all 7 grasp features as input to the classifier, we use only \textit{one}. 
For each pair of primitive and performance metric, we identify the most important feature according to the results in Fig.~\ref{fig:imps} (e.g., for cylinder primitives and the maximum stress metric, $edge\_dist$ is most important). Whenever this important feature is \textit{correlated} with the performance metric, we assume that this feature-metric pair is \textit{also correlated} on unseen objects geometrically similar to the associated primitive, where object similarities are informed by whether they belong to the same category in Fig.~\ref{fig:object_categories}. For example, if $edge\_dist$ and maximum stress are correlated among grasps on a cylinder, we hypothesize that they will also be correlated among grasps on a banana, which is cylinder-like. We then rank the grasps according to the value of the grasp feature and use this ordering as a direct prediction of the rank of the grasps according to the value of the performance metric. Using this method, we predict the 5 grasps that will yield the highest metric values, and we define a prediction as \textit{accurate} if it belongs to the set of grasps that actually yield the top 15 metric values (i.e., the top 30th percentile for 50 total grasps). The same method is used to predict the 5 grasps that yield the lowest metric values. We now highlight some successful examples of this approach on unseen objects. In the following figures, the line representation of the gripper pose will be used (see Fig. \ref{fig:qm}\subref{fig:skeleton}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-8pt}
\subsection{Predicting Maximum Stress on Spheroid-like Objects}
On the spheroid primitives, $pure\_dist$ is most important for classifying maximum stress ($R{=}0.84$) (Fig.~\ref{fig:imps}b). This correlation generalizes to other spheroid-like objects like a lemon, apple, and peach ($R{=}0.72, 0.72, 0.68$). We demonstrate prediction on a heart due to its asymmetry and surgical significance. Of the 10 predictions, 9 are accurate (Fig.~\ref{fig:heart_5}).
% we predict the grasps with the lowest and highest maximum stress values (Fig. \ref{fig:heart_5}a) and find that 9 of 10 predictions are accurate (Fig. \ref{fig:heart_5}b). 
We visualize the stress distribution of the one grasp incorrectly predicted to be low-stress in Fig.~\ref{fig:heart_examples}b. As depicted, the gripper finger contacts small protrusions on the heart that reduce contact area and increase the maximum stress. These local protrusions are not captured by the $pure\_dist$ feature, as it does not quantify contact patch shape. This suggests that other features such as $num\_contacts$ should also be considered.

% Combining $pure\_dist$ with other features such as $num\_contacts$ could further ensure that all predictions are accurate.

\begin{figure}
\captionsetup{width=0.45\columnwidth}
\centering
\begin{minipage}{.5\columnwidth}
  \centering
     \begin{subfigure}[b]{.4\columnwidth}
         \centering
         \includegraphics[scale=0.12, trim={22cm 18cm 26cm 12cm},clip]{real_objects/heart_predicted.png}
         \caption{Predicted.}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{.4\columnwidth}
         \centering
         \includegraphics[scale=0.12, trim={22cm 18cm 27cm 12cm},clip]{real_objects/heart_actual.png}
         \caption{Actual.}
     \end{subfigure}
        \caption{Lowest (green) and highest-valued (orange) five heart grasps for max stress.}
        \label{fig:heart_5}
\end{minipage}%
\begin{minipage}{.5\columnwidth}
     \begin{subfigure}[b]{.38\columnwidth}
         \centering
         \includegraphics[scale=0.09, trim={2cm 0cm 7.5cm 0cm},clip]{real_objects/heart_low_example2.png}
         \caption{Accurate.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{.47\columnwidth}
         \centering
         \includegraphics[scale=0.09]{real_objects/heart_real.png}
         \caption{Inaccurate.}
     \end{subfigure}
        \caption{Examples of predicted low stress grasps.}
        \label{fig:heart_examples}
\end{minipage}
\vspace{-18pt}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-6pt}
\subsection{Predicting Max Deformation on Container-like Objects}
On the cup and flask, $squeeze\_dist$ is correlated with maximum deformation ($R{=}0.89$ for cup, $R{=}0.93$ for flask). This generalizes to a tall cup, a mug, a mustard bottle, and a bleach bottle ($R{=}0.89, 0.84, 0.77, 0.76$), on which all 40 predicted grasps are accurate (Fig.~\ref{fig:containers}). On the tall cup, the predicted lowest-valued grasps (i.e., for maximum deformation) are concentrated at the base, and the predicted highest-valued grasps are concentrated at the lip (Fig. \ref{fig:containers}a). On the mug, the lowest-valued grasps are those that are top-bottom grasps since its height fits within the gripper opening, unlike with the tall cup. The highest-valued grasps all contact the handle of the mug, which buckles severely when squeezed (Fig. \ref{fig:containers}b). On the bottles, low-valued grasps mostly squeeze at the base where local stiffness is higher, and high-valued grasps squeeze the bottle faces, inducing maximal buckling (Fig. \ref{fig:containers}cd). 
% Example deformation fields are in Fig.~\ref{fig:mustard_examples}.

% \YN{In case there is time and space... Were there any other interesting cases of generalization?} 

\begin{figure}
     \centering
     \begin{subfigure}[b]{.24\columnwidth}
         \centering
         \includegraphics[scale=0.17, trim={0cm 0cm 33.5cm 0cm},clip]{real_objects/containers.png}
         \caption{Tall cup.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{.24\columnwidth}
         \centering
         \includegraphics[scale=0.17, trim={11cm 0cm 21cm 0cm},clip]{real_objects/containers.png}
         \caption{Mug.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{.24\columnwidth}
         \centering
          \includegraphics[scale=0.17, trim={24cm 0cm 11cm 0cm},clip]{real_objects/containers.png}
         \caption{Mustard bottle.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{.24\columnwidth}
         \centering
          \includegraphics[scale=0.17, trim={34cm 0cm 0cm 0cm},clip]{real_objects/containers.png}
         \caption{Bleach bottle.}
     \end{subfigure}
        \caption{Predicted lowest (green) and highest-valued (orange) five grasps on containers for maximum deformation.}
        \label{fig:containers}
\vspace{-15pt}
\end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Predicting Max Deformation on Hollow Flask-like Objects}
% We test the predictive power of $squeeze\_dist$ on deformation-based metrics due to its leading importance in classifying grasps with respect to deformation for the flask primitive (Fig. \ref{fig:imps}e). There is a positive correlation between $squeeze\_dist$ and maximum deformation on the flask ($R{=}0.93$) that generalizes to a mustard bottle ($R{=}0.77$) and a bleach bottle ($R{=}0.76$). The predicted five lowest and highest-valued grasps for maximum deformation on a mustard bottle are in Fig. \ref{fig:mustard_grasps}\subref{fig:mustard_pred}, with the ground truth grasps depicted in Fig. \ref{fig:mustard_grasps}\subref{fig:mustard_low_acc}\subref{fig:mustard_high_acc}. All predictions were accurate, and examples of the deformation fields induced by these predicted grasps are in Fig. \ref{fig:mustard_examples}. 

% \begin{figure}[H]
% \centering
% \includegraphics[scale=0.3]{real_objects/squeeze_vs_def.png}
% \caption{$squeeze\_dist$ vs max. def. for multiple closed hollow containers/}
% \label{fig:shaking_scatter}
% \end{figure}


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{.25\columnwidth}
%          \centering
%          \includegraphics[scale=0.12, trim={22cm 16cm 22cm 11cm},clip]{mustard/mustard_pred.png}
%          \caption{Predicted.}
%          \label{fig:mustard_pred}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.35\columnwidth}
%          \centering
%          \includegraphics[scale=0.12, trim={22cm 16cm 22cm 11cm},clip]{mustard/actual_min_mustard.png}
%          \caption{Actual lowest def.}
%          \label{fig:mustard_low_acc}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.35\columnwidth}
%          \centering
%          \includegraphics[scale=0.12, trim={20cm 16cm 19cm 11cm},clip]{mustard/actual_mustard_high.png}
%          \caption{Actual highest def.}
%          \label{fig:mustard_high_acc}
%      \end{subfigure}
%         \caption{Lowest (green) and highest-valued (orange) five grasps for max. deformation on a mustard bottle.}
%         \label{fig:mustard_grasps}
% \end{figure}


%% TEMPORARILY GOT RID OF THIS
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{.23\columnwidth}
%          \centering
%          \includegraphics[scale=0.08, trim={6cm 0cm 9cm 0cm},clip]{mustard/low1.png}
%          \caption{}
%          \label{fig:mustard_low1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.23\columnwidth}
%          \centering
%          \includegraphics[scale=0.08, trim={6cm 0cm 0cm 0cm},clip]{mustard/high1.png}
%          \caption{}
%          \label{fig:mustard_low2}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.23\columnwidth}
%          \centering
%          \includegraphics[scale=0.08, trim={6cm 0cm 9cm 0cm},clip]{figures/bleach/low_def.png}
%          \caption{}
%          \label{fig:mustard_high1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.23\columnwidth}
%          \centering
%          \includegraphics[scale=0.08, trim={6cm 0cm 0cm 0cm},clip]{figures/bleach/high_def.png}
%          \caption{}
%          \label{fig:mustard_high2}
%      \end{subfigure}
%         \caption{Examples of accurate low and high-valued maximum deformation predictions using the $squeeze\_dist$ feature on (ab) a mustard bottle and (cd) bleach bottle. \IH{should I get rid of this?}}
%         \label{fig:mustard_examples}
% \vspace{-18pt}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% \subsection{Predicting Def. Controllability on Cylinder-like Objects}
% Deormation controllability is a metric strongly correlated with the $perp\_dist$ features ($R{=}0.78$). Using $perp\_dist$ as the predictive feature, we generated all accurate predictions of the lowest and highest-valued five grasps for controllability on a banana (Fig. \ref{fig:banana_grasps}\subref{fig:banana_pred}). An example of an accurate high controllability grasp is shown in Fig. \ref{fig:banana_grasps}\subref{fig:banana_actual}.


% % \YN{In these subsections, various performance metrics are discussed -- sometimes stress, sometimes controllability, etc. A critical reviewer may wonder, what happened for the metrics that are *not* being discussed for a particular object? Were the results also good for those, or are they not being presented because they were not good? If the results were reasonably good, it may be useful to say that, to defend against this critique; and you can still do as you're doing now, i.e., only presenting the results in detail for the most interesting metrics}
% \begin{figure}[H]
%      \centering
%      \begin{subfigure}[b]{.4\columnwidth}
%          \centering
%          \includegraphics[scale=0.12, trim={13cm 16cm 17cm 11cm},clip]{real_objects/banana_predict.png}
%          \caption{}
%          \label{fig:banana_pred}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{.5\columnwidth}
%          \centering
%          \includegraphics[scale=0.11, trim={0cm 0cm 0cm 0cm},clip]{figures/banana/high_ctrl.png}
%          \caption{}
%          \label{fig:banana_actual}
%      \end{subfigure}
%         \caption{(a) Predicted lowest (green) and highest-valued (orange) five grasps for deformation controllability on a banana, (b) example of a predicted high-valued grasp.}
%         \label{fig:banana_grasps}
% \end{figure}
